Do Large Language Models Understand Performance Optimization?

Large Language Models (LLMs) have emerged as powerful tools for software development tasks such as code completion, translation, and optimization. However, their ability to generate efficient and correct code, particularly in complex High-Performance Computing (HPC) contexts, has remained underexplored. To address this gap, this paper presents a comprehensive benchmark suite encompassing multiple critical HPC computational motifs to evaluate the performance of code optimized by state-of-the-art LLMs, including OpenAI o1, Claude-3.5, and Llama-3.2. In addition to analyzing basic computational kernels, we developed an agent system that integrates LLMs to assess their effectiveness in real HPC applications. Our evaluation focused on key criteria such as execution time, correctness, and understanding of HPC-specific concepts. We also compared the results with those achieved using traditional HPC optimization tools. Based on the findings, we recognized the strengths of LLMs in understanding human instructions and performing automated code transformations. However, we also identified significant limitations, including their tendency to generate incorrect code and their challenges in comprehending complex control and data flows in sophisticated HPC code.

==> backup/author.tex <==
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
% \author{Ben Trovato}
% \authornote{Both authors contributed equally to this research.}
% \email{trovato@corporation.com}
% \orcid{1234-5678-9012}
% \author{G.K.M. Tobin}
% \authornotemark[1]
% \email{webmaster@marysville-ohio.com}
% \affiliation{%
%   \institution{Institute for Clarity in Documentation}
%   \city{Dublin}
%   \state{Ohio}
%   \country{USA}
% }

% \author{Lars Th{\o}rv{\"a}ld}
% \affiliation{%
%   \institution{The Th{\o}rv{\"a}ld Group}
%   \city{Hekla}
%   \country{Iceland}}
% \email{larst@affiliation.org}

% \author{Valerie B\'eranger}
% \affiliation{%
%   \institution{Inria Paris-Rocquencourt}
%   \city{Rocquencourt}
%   \country{France}
% }

==> backup/bg.tex <==
\section{Background and Related Work} \Outline{0.5 page}

\paragraph{LLMs for Code}

Large Language Models (LLMs) for code generation utilize natural language descriptions, such as programming problem statements or docstrings, to produce source code~\cite{jiang2024surveylargelanguagemodels}. These models have been trained on vast datasets that include a wide variety of programming languages and application domains. This extensive training enables LLMs to understand and generate code that aligns with the intent expressed in natural language inputs. Additionally, LLMs designed for code tasks typically undergo pre-training on large corpora like The Stack~\cite{stack}, which includes open-source code, or The Pile~\cite{pile}, which aggregates diverse text data, including code. Some models, such as CodeLlama~\cite{codellama}, are initially trained as general-purpose language models and later fine-tuned on specialized code datasets to enhance their coding capabilities~\cite{jiang2024surveylargelanguagemodels}. However, generating high-quality code from LLMs requires careful handling to avoid issues like repetition or low-quality outputs. Techniques such as nucleus sampling and temperature adjustment are commonly used to manage the diversity and quality of the generated code~\cite{meteor}.

The practical application of these models has led to the development of advanced coding assistants. Tools like GitHub Copilot, powered by OpenAI's Codex~\cite{gitcopilot}, provide real-time code suggestions and completions within integrated development environments (IDEs), significantly enhancing developer productivity. Similarly, CodeGeeX~\cite{codegeex} and Amazon's CodeWhisperer~\cite{codewhisperer} offer features such as code completion, translation, and comment generation, making them invaluable assets in modern software development workflows.

\paragraph{Traditional Code Optimization Tools}

Before the emergence of LLMs, there were some traditional code optimization tools. For examples, MAQAO~\cite{MAQAO} achieves performance analysis and optmization by parsing assembly code to build structured representations, allowing detailed static and dynamic analyses, code pattern detection, and targeted optimizations specifically tailored for HPC applications. KBS-MAQAO~\cite{KBS-MAQAO} builds upon the MAQAO framework by incorporating a Knowledge Based System (KBS) that includes a Descriptive Model (DM) and a Knowledge Base (KB). This system enhances optimization effiency and quality by guiding users to improve performance and/or code quality with minimal interaction, while avoiding redundant processes on identical loops. HPCTOOLKIT~\cite{hpctookit} analyzes the performance of complex HPC applications by collecting detailed measurements through sampling, attributing performance metrics to the full calling context, and identifying inefficiencies such as load imbalance, synchronization bottlenecks, and poor memory hierarchy utilization.

\paragraph{Codee}

==> backup/challenges.tex <==
% Automatic Parallelization is challenging
Optimizing and parallelizing HPC applications has long been a complex and manual-intensive task. Efforts by the compiler community to automate parallelization have met with only partial success, primarily due to challenges in dependence analysis, inter-procedural analysis, alias analysis, and the profitability estimation of the parallel codes done statically. These challenges are compounded by the intricacies of parallel computations, where bugs like race conditions and synchronization errors often surface only at runtime, especially as applications scale to multiple compute units. To avoid this issues, compilers tend to be conservative for their parallel code transformations.

%Highlight opportunities for LLMs but also the challenges
Using LLMs to parallelize codes means that the generated code needs to satisfy dependences and the limited availability of large, representative corpora for training machine learning models on parallel optimizations - compared to the abundance of datasets for serial optimizations—further can be challenging in this area.  
%A challenge for LLMs is introduction of bugs that passes test because they dont show up in test coditions
Another significant challenge is the presence of parallel bugs that exhibit the Heisenberg effect, where a race condition may exist despite the code producing correct results under certain test conditions. These bugs may only manifest as the application scales or runs on different architectures, making them particularly elusive. 

%Explainability is key and a step forward
Given these complexities, there is a pressing need to understand how LLMs recognize and address parallel optimization challenges and to assess the potential risks that might arise in large-scale applications. 

%And integrated approach to check for correctness of code produced by LLMs is important
An integrated approach that combines advanced analysis tools with rigorous correctness verification mechanisms could enhance the reliability of optimizations while minimizing the introduction of new bugs in HPC applications. This approach warrants a thorough exploration, given its potential to bridge the gaps between current compiler capabilities and the rapid advances of LLMs.


==> backup/modify.tex <==
Note that: Experiments were conducted by two graduate students with limited background in HPC code optimization. The code and benchmark results have been verified by several experienced performance engineers. 

We establish five experiments to analyze the performance of \textit{Codee}, \textit{ChatGPT-4}, and \textit{Llama3.1}. Note that, when analyzing code, \textit{Codee} may identify multiple checkers and assign a priority level to each based on the significance of the optimization to the program. These priority levels are ranked from highest to lowest as \textit{L1}, \textit{L2}, and \textit{L3}. 
\begin{itemize}
    \item For Experiment 1: Serial Optimization (\ref{sub:EX1}, denoted EX1), we focused solely on serial optimization (serial checkers) in \textit{Codee} and selected a single \textit{L1} checker for optimization. For the LLMs, we apply the prompt mentioned in \autoref{framework} for EX1 directly to optimize the code.
    \item For Experiment 2: Multiple Rounds of Serial Optimization (\autoref{sub:EX2}, denoted EX2), we optimize all \textit{L1} checkers and selected some \textit{L2} and \textit{L3} checkers in \textit{Codee}, while in the LLMs, we re-optimize the code already optimized in EX1 using the prompt outlined in \autoref{framework} for EX2.
    \item For Experiment 3: Parallel Optimization (\autoref{sub:EX3}, denoted EX3), our focus in \textit{Codee} is exclusively on parallel optimization (parallel checkers), and we use the EX3 prompt from \autoref{framework} directly for the LLMs.
    \item For Experiment 4: Time Spent on Applying Optimization (\autoref{sub:EX4}, denoted EX4), it measures the time required, from the start of optimization to successful compilation and execution, for the optimized code generated bu the three approaches (\textit{Codee}, \textit{ChatGPT-4}, and \textit{Llama3.1}) across EX1, EX2, and EX3.
    \item For Experiment 5: Correctness (\autoref{subsec:EX5}, denoted EX5), it assesses the correctness of the compiled results for the optimized code from these experiments. Note that: we use the \textit{pass@1} to represent correctness, which means 
    \item For Experiment 6: Explainability (\autoref{subsec:EX6}, denoted EX6), it evaluates the explanation quality of the optimized code gnerated by each approach. Typically, \textit{Codee} provides reasons for optimizations during code inspection, while LLMs may or may not do so. If the LLMs do not provide explanations directly, we prompt them with, "Give me some explanations for the optimizations you made."
\end{itemize}

Additionally, for all optimized codes generated in EX1, EX2, and EX3, we measure and compare the runtime (averaged over 10 runs, except for susan, which is averaged over 10 sets of 100 runs) against the original code.

==> src/RelatedWork.tex <==
\section{Related Work}
\label{sec:related work}
\noteboxbowen{
1. Add citations

2. Simplify the description. For each related work you just need to use 1-2 sentences to describe it.
}
\paragraph{LLMs for Code.} LLMs have achieved remarkable progress in automated code generation, primarily through instruction tuning, where models are trained on curated datasets of prompts and code outputs~\cite{jiang2024surveylargelanguagemodels}. 
Reinforcement learning with human feedback (RLHF)~\cite{ouyang2022traininglanguagemodelsfollow} further refines their ability to generate syntactically and functionally correct code, with models like CodeRL~\cite{NEURIPS2022_8636419d} and PPOCoder~\cite{shojaee2023executionbasedcodegenerationusing} demonstrating substantial improvements on benchmarks such as HumanEval. 
Additionally, prompt engineering techniques, such as Chain-of-Thought~\cite{wei2023chainofthoughtpromptingelicitsreasonin} and Self-Debugging~\cite{chen2023teachinglargelanguagemodels}, enable iterative refinements, while retrieval-augmented generation (RAG) addresses the complexity of repository-level code generation by incorporating cross-file context, as seen in frameworks like RepoCoder~\cite{zhang2023repocoderrepositorylevelcodecompletion}.

\paragraph{LLMs for HPC.}

\paragraph{Evaluating LLMs.} Evaluating LLMs in code generation employs metrics-based, human-centered, and LLM-based approaches~\cite{jiang2024surveylargelanguagemodels}. 
For metrics-based methods, they measure correctness and similarity of generated codes with the reference codes, such as BLEU~\cite{Papineni2002BleuAM}, ROUGE~\cite{lin-2004-rouge}, and METEOR~\cite{banerjee-lavie-2005-meteor}, which often fail to adequately capture the syntactic and functional correctness of generated codes.
Although there exists some sophisticated metrics like CodeBLEU~\cite{ren2020codebleumethodautomaticevaluation} which incorporates abstract syntax trees (AST) and data-flow graphs (DFG), they still fall short of evaluating execution-based correctness.
As a result, execution-based metrics, such as pass@k~\cite{Evauating_LLMs_Trained_on_Code} and execution accuracy~\cite{rajkumar2022evaluatingtexttosqlcapabilitieslarg}, have gained prominence as they directly assess the functional validity of generated code through unit tests.
Additionally, Human-centered evaluation captures qualitative aspects such as style and maintainability but is resource-intensive and subject to bias~\cite{jiang2024surveylargelanguagemodels}. 
Lastly, LLM-based evaluation, exemplified by "LLM-as-a-Judge," offers scalable solutions with interpretability but faces challenges due to model biases~\cite{jiang2024surveylargelanguagemodels}. 

\paragraph{LLM Agents}.
%Combining these approaches is essential to developing robust and reliable evaluation frameworks for automated code generation.

==> table/tabl4-1_opt_list.tex <==
\begin{table*}[t]
\centering
\scriptsize
\caption{Summary of Optimizations Applied}
\label{tab:Optimization-list}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Optimization}   & \textbf{Codee}        & \textbf{Open AI o1}   & \textbf{Llama-3.2}     & \textbf{Claude-3.5} \\ \hline
Loop Reordering    &        1               &   8                   &       1                &                   \\ \hline
Loop Unrolling     &                       &    6                   &      3                 &             5      \\ \hline
Loop Tiling        &                       &    2                   &    1                   &           1        \\ \hline
Loop Fission       &       2                &                       &     1                  &                   \\ \hline
Loop Fusion       &                       &    2                   &    1                   &       7            \\ \hline
Memory optimization &                      &          8             &        13               &           10       \\ \hline
Cache Blocking     &                       &                       &       1                &                   \\ \hline
Pre-Computing Constants &                 &            6           &         2              &                5   \\ \hline
Fused Multiply-Add &               13       &                       &                       &                   \\ \hline
Change of Precision &          3           &                       &                       &                   \\ \hline
Mathematical Simplification &          6    &         3              &          7             &    18      \\ \hline
Reducing Function Overhead &              &         4              &         3              &                   \\ \hline
OpenMP Scoping     &        1               &     5                  &     5                 &           5        \\ \hline
OpenMP Vectorization &          7          &          18             &         11             &              10     \\ \hline
OpenMP Reduction   &        3               &      9                 &      3                 &          4         \\ \hline
SIMD optimizations &                       &          2             &        1               &          3         \\ \hline
\end{tabular}
\end{table*}


==> table/table4_opt_list.tex <==
[TAB 4] What optimizations have been applied and whether LLMs explain their optimization correctly
\begin{table}[h!]
\centering
\caption{Summary of Optimizations Applied\tablefootnote{LN = Loop Nesting, LR = Loop Reordering, LU = Loop Unrolling, LT = Loop Tiling, LF = Loop Fission, LFU = Loop Fusion, MO = Memory Optimization, CB = Cache Blocking, PCC = Pre-Computing Constants, FMA = Fused Multiply-Add, COP = Change of Precision, MS = Mathematical Simplification, RFO = Reducing Function Overhead, ATT = \_\_attribute\_\_(pure), MT=Multithreading OV = OpenMP Scoping, OV = OpenMP Vectorization, OR = OpenMP Reduction, SI=SIMD Optimizations.}}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l l l}
  \midrule
  Tool     & Example        & Optimization Applied  \\
  \midrule
  Codee    & MATMUL         & LI,FMA,MT                \\
  ChatGPT-4    & MATMUL         & LI,LU,CB,MS           \\
  Llama3.1 & MATMUL         & LI,LU,CB              \\
  Codee    & ATMUX          & LF,FMA,MT                \\
  ChatGPT-4    & ATMUX          & LFU,MO,PCC,RFO        \\
  Llama3.1 & ATMUX          & LU,MO,CB,MS           \\
  Codee    & PI             & MS,MT                    \\
  ChatGPT-4    & PI             & LU,PCC,COP,OR            \\
  Llama3.1 & PI             & LU,CB,COP,MS,OR          \\
  Codee    & CANNY          & FMA,COP,MS,ATT,MT        \\
  ChatGPT-4    & CANNY          & LU,MO,RFO,OR,OS           \\
  Llama3.1 & CANNY          & OR,OS                   \\
  Codee    & COULOMB        & FMA,MS,MT                \\
  ChatGPT-4    & COULOMB        & LU,PCC,MS             \\
  Llama3.1 & COULOMB        & LU,MO,CB,PCC,RFO      \\
  Codee    & HACCmk         & MT,FMA,MS                   \\
  ChatGPT-4    & HACCmk         & MT,OR,MO                      \\
  Llama3.1 & HACCmk         & OR,MT                     \\
  Codee    & NPB\_CG        & MT,LF,FMA                   \\
  ChatGPT-4    & NPB\_CG        & MT,OR                   \\
  Llama3.1 & NPB\_CG        & OR,RFO                    \\
  Codee    & Hotspot        & FMA,COP,OS,MT          \\
  ChatGPT-4    & Hotspot        & LU,MO,CB,PCC,MS       \\
  Llama3.1 & Hotspot        & LI,LU,MO,CB,RFO        \\
  Codee    & Hotspot3D      & MO,FMA,COP,MS,ATT,OS,OV \\
  ChatGPT-4    & Hotspot3D      & LI,LU,MO,COP,RFO      \\
  Llama3.1 & Hotspot3D      & LU,CB                 \\
  Codee    & Particlefilter & LF,MO,FMA,MS,ATT,OS,OV  \\
  ChatGPT-4    & Particlefilter & LI,LU,MO,RFO,OR      \\
  Codee    & Srad           & LF,FMA,COP,OS,OV       \\
  ChatGPT-4    & Srad           & LU,LT,MO,COP,OR      \\
  Llama3.1 & Srad           & LU,MO,RFO,OR        \\
  Codee    & Qsort          & MS,ATT                      \\
  ChatGPT-4    & Qsort          & MS,RFO,MO                    \\
  Llama3.1 & Qsort          & MS,RFO,LU,CB,SI                     \\
  Codee    & Sha            & OV,                     \\
  ChatGPT-4    & Sha            & LU,MO,RFO                      \\
  Llama3.1 & Sha            & LU,SI,MO                      \\
  Codee    & Susan          & OV,ATT,COP                     \\
  Codee    & FFT            & COP,FMA                      \\
  ChatGPT-4    & FFT            & MS,MO,LU,RFO                      \\
  Llama3.1 & FFT            & RFO,MO,LU,CB,SI                     \\
  \midrule
\end{tabular}
}
\label{tab:Optimization-list}
\end{table}


==> todo.tex <==
\newcommand{\todoc}[2]{{\textcolor{#1}{\textbf{#2}}}}

\newcommand{\todored}[1]{{\todoc{red}{\textbf{[[#1]]}}}}
\newcommand{\todogreen}[1]{\todoc{green}{\textbf{[[#1]]}}}
\newcommand{\todoblue}[1]{\todoc{blue}{\textbf{[[#1]]}}}
\newcommand{\todoorange}[1]{\todoc{orange}{\textbf{[[#1]]}}}
\newcommand{\todobrown}[1]{\todoc{brown}{\textbf{[[#1]]}}}
\newcommand{\todogray}[1]{\todoc{gray}{\textbf{[[#1]]}}}
\newcommand{\todopink}[1]{\todoc{pink}{\textbf{[[#1]]}}}
\newcommand{\todopurple}[1]{\todoc{purple}{\textbf{[[#1]]}}}
\newcommand{\todo}[1]{\todored{TODO: #1}}
\newcommand{\TODO}[1]{\todored{TODO: #1}}

%% To disable colored comments, just uncomment this line: 
%\renewcommand{\todoc}[2]{\relax}

%----------- Comment command for each person ------------
\newcommand{\Keren}[1]{\todored{Keren: #1}}
\newcommand{\Bowen}[1]{\todoorange{Bowen: #1}}
\newcommand{\Tejas}[1]{\todoblue{Tejas: #1}}
\newcommand{\Outline}[1]{\todopurple{#1}}
